Consistency pays off in science

The exponentially growing number of scientific papers stimulates a discussion on the interplay between quantity and quality in science. In particular, one may wonder which publication strategy may offer more chances of success: publishing lots of papers, producing a few hit papers, or something in between. Here we tackle this question by studying the scientific portfolios of Nobel Prize laureates. A comparative analysis of different citation-based indicators of individual impact suggests that the best path to success may rely on consistently producing high-quality work. Such a pattern is especially rewarded by a new metric, the $E$-index, which identifies excellence better than state-of-the-art measures.

==> Citation inequalities/preamble.tex <==
% \usepackage[round,authoryear]{natbib}
%Add here your packages or commands
\usepackage[svgnames,usenames,dvipsnames]{xcolor}
\usepackage{lipsum}
\usepackage{colortbl}
 \usepackage{booktabs}
 \usepackage{multirow}
 \usepackage{graphicx,bigdelim}

\usepackage{comment}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{pgfplots.groupplots,arrows,automata,positioning}
\usepgfplotslibrary{dateplot,fillbetween}
% \selectcolormodel{cmyk}
\usepgfplotslibrary{dateplot}
\pgfplotsset{compat=newest}
\usetikzlibrary{spy}

\pgfplotsset{every axis/.append style={
                    % xlabel={$x$},          % default put x on x-axis
                    % ylabel={$y$},          % default put y on y-axis
                    label style={font=\sffamily\large},
                    tick label style={font=\sffamily\scriptsize},
                    title style = {font=\sffamily\large},
                    ylabel near ticks,
                    y label style={font=\sffamily\large},
                    xlabel near ticks,
                    x label style={font=\sffamily\large},
                    legend cell align={left},
                    legend style={draw=none, font=\sffamily\normalsize},
                    },
                    legend image code/.code={
                    \draw[mark repeat=2,mark phase=2]
                        plot coordinates {
                        (0cm,0cm)
                        (0.15cm,0cm)        %% default is (0.3cm,0cm)
                        (0.3cm,0cm)         %% default is (0.6cm,0cm)
                        };%
                    },
                    boxplot/hide outliers/.code={
                        \def\pgfplotsplothandlerboxplot@outlier{}%
                    }
                    }
\pgfplotsset{compat=newest}  
\pgfplotsset{
    jitter/.style={
        x filter/.code={\pgfmathparse{\pgfmathresult+(rnd-.5)*#1}}
    },
    jitter/.default=0.1
}


% argument #1: any options
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%
% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}


% We will externalize the figures
% \usepgfplotslibrary{external}
% \tikzexternalize

%%%% *** Do not adjust lengths that control margins, column widths, etc. ***

%%%%%%%%%%% Defining Enunciations  %%%%%%%%%%%
\newtheorem{theorem}{\bf Theorem}[section]
\newtheorem{condition}{\bf Condition}[section]
\newtheorem{corollary}{\bf Corollary}[section]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\satyaki}[1]{(\textcolor{blue}{Satyaki}: \textit{#1})}
\newcommand{\rank}[1]{ \tiny{\textsuperscript{(#1)}}}

\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\etal}{\textit{et al.}}
\newcommand{\para}[1]{\textbf{#1}.\quad}
% \newcommand{\para}[1]{}
